PIVOT: Prompting for Video Continual Learning

Modern machine learning pipelines are limited due to data availability, storage quotas, privacy regulations, and expensive annotation processes. These constraints make it difficult or impossible to train and update large-scale models on such dynamic annotated sets. Continual learning directly approaches this problem, with the ultimate goal of devising methods where a deep neural network effectively learns relevant patterns for new (unseen) classes, without significantly altering its performance on previously learned ones. In this paper, we address the problem of continual learning for video data. We introduce PIVOT, a novel method that leverages extensive knowledge in pre-trained models from the image domain, thereby reducing the number of trainable parameters and the associated forgetting. Unlike previous methods, ours is the first approach that effectively uses prompting mechanisms for continual learning without any in-domain pre-training. Our experiments show that PIVOT improves state-of-the-art methods by a significant 27% on the 20-task ActivityNet setup.

==> sections/3_method_backup.tex <==
\section{Prompting for Video Continual Learning}\label{sec:method}

\begin{figure*}[t]
    % \vspace{-1.2cm}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/img_model.pdf}
    % \vspace{-3mm}
    \caption{
    \textbf{Outline of the PIVOT Model at inference time.} Our model follows 3 main stages to make a prediction in video CIL setup: \textbf{(1)} PIVOT selects the specific task prompts for a video instance based on its similarity with the keys $K$ of each task prompt (Blue box). \textbf{(2)} Then, PIVOT adds the selected spatial and temporal task prompts to the corresponding encoder spatial (CLIP) or Temporal Encoder (green box). \textbf{(3)} Finally, PIVOT classifies the video following an MCL, considering the similarity with text embeddings from the labels of all the available classes computed with the CLIP text encoder (black box).
    }
    \vspace{-4mm}
    \label{fig:model_fig}
\end{figure*}

% \textcolor{red}{\textbf{Motasem is holding the token for this section}}

Our main objective is to leverage the knowledge available in large-scale image-language models for video CIL. That is, we want to learn how to adapt large visual-language DNNs available in the image domain into a single end-to-end network that is effective in video CIL. Furthermore, we want to make sure that such a transfer of knowledge involves no fine-tuning of the image encoder, and requires minimal extensions over the original network. Such constraints will ultimately favor less forgetting in the CIL setup, as the key parameters will suffer less drift during fine-tuning on different tasks. 


Our approach, PIVOT, is divided into three major components.
\textbf{(i)} We adapt a large-scale image-language pre-trained model, CLIP \cite{clip}, to extract visual information from video data.
\textbf{(ii)} We aggregate the temporal information extracted from several frames within a video via a transformer encoder.
\textbf{(iii)} We reinforce the learned knowledge from each task by deploying learnable tokens, \ie prompts, to prevent the forgetting of previously learned tasks.
Despite its multiple components, we train PIVOT in an end-to-end fashion. We highlight that this training process is lightweight since the image and text encoders are frozen.
Before we delve into the details of each of our model components, we give a brief preliminary on the Video Class Incremental Learning~(VCIL) problem and the multi-modal contrastive classifier proposed in CLIP, as it plays a key role in our approach. 

% First, we propose a strategy to adapt an image knowledge-base to work on the visual targets found in the video domain, \textbf{i.e.} we modify the knowledge base to perform single frame video action recognition instead of image classification. Second, we adapt a transformer layer to handle the modeling of temporal information, this information is exclusive of the video-domain and can not be found in any image knowledge-base. Third, we train the image knowledge base and the transformer in an end-to-end fashion. The resulting model, named PIVOT (PromptIng in VideO conTinual learning), can out-perform every other video CIL method, despite having no in-domain pre-training and tuning a single component on it, namely a 3-layer temporal transformer.

\subsection{Problem Definition}
We follow the recent vCLIMB benchmark~\cite{Villa_2022_CVPR} training a single model $f_\theta: \mathcal X \rightarrow \mathcal Y$, \ie a DNN parameterized with $\theta$, that learns to predict an action label $y\in\mathcal{Y}$ given an input video $x\in\mathcal{X}$. The model learns from a sequence of tasks $\{(X_1, Y_1),(X_2, Y_2),\dots,(X_n, Y_n)\}$ where $X_i\in\mathcal X$ and $Y_i \in \mathcal Y \,\,\forall i$.
In the class-incremental setup, we assume that different tasks present the model with a different set of labels, \ie $Y_i \cap Y_j = \emptyset \,\,\forall i\neq j$.
We define $Acc_i$ as the average classification accuracy of all the tasks up to and including task $i$. Our objective is to train a single model $f_\theta$ that maximizes the average accuracy $Acc$, which is the average over all $Acc_i$.


\subsection{Multi-modal Contrastive Classifier for Video Continual Learning}\label{sec:mcl}

%%%%%%%%%%%%%%% Mota Version %%%%%%%%%%%%%%%
% Our method builds on top of the large pretrained CLIP encoder.
% Hence, to utilize CLIP for VCIL, we deploy a multi-modal contrastive classifier for the extracted features. 
% We first use CLIP's textual encoder to extract text embeddings for the labels of all the observed classes.
% Then, to classify a given video, we choose the class that minimizes the distance between the textual embedding for the label and the visual embeddings for the video frames.
% We note here that we employ an average pooling layer to aggregate the visual information for several frames of a given video. \AV{This is confusing. We use a transformer encoder to aggregate temporal information in our model}

% We observe the following advantages of our Multi-modal Contrastive Learning~(MCL) for the continual learning setup.
% First, this approach is parameter-free.
% Therefore, our classifier would not suffer from \emph{any} forgetting when learning different tasks.
% This mitigates the need to deploy a replay buffer to maintain the performance of the classifier on previously learnt tasks.
% Second, this approach allows for directly leveraging a frozen CLIP encoder in the VCIL setup in a zero-shot fashion without the need to add any other module.
% We found experimentally in Section~\ref{sec:results} that, despite the simplicity of this approach, a zero-shot CLIP significantly outperforms all continual learning methods in the literature on the Kinetics and ActivityNet VCIL setups.
% Next, we discuss our approach that builds on top of the frozen CLIP encoder.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Our method builds on top of the image-language pre-trained CLIP encoder. CLIP \cite{clip} demonstrated that textual information promotes the learning of transferable visual features. PIVOT re-purposes the CLIP encoder for video CIL by using its multi-modal contrastive classifier as a video feature generator. We use CLIP's language encoder to extract text embeddings from the labels of all the available classes, and  its image encoder to extract visual embeddings for arbitrary frame data. These paired embeddings allow us to perform a pseudo-classification by looking for tuples that minimize the distance between visual and textual embeddings. By keeping the CLIP's encoder frozen and forwarding video related data (in the visual and language streams), we allow the transfer of its extensive knowledge into the video domain in a zero-shot fashion. 
% \fch{zero-shot classification (?)}
%Remarkably, such an approach involves no parameter tuning, thereby avoid any forgetting along arbitrary long task sets on the CL setup. 
%, and \cite{tnt} outlined that it helps to learn with few examples.

We observe three advantages in Multi-modal Contrastive Learning~(MCL) for the continual learning setup.
First, this approach is parameter-free. Hence, our classifier would not suffer from \emph{any} forgetting when learning different tasks.
This mitigates the need to deploy a large replay buffer to maintain the performance of the classifier on previously learned tasks.
Second, this approach directly leverages the frozen CLIP encoder in the video CIL setup.
%herefore, for the zero-shot CLIP, we employ an average pooling layer to aggregate the visual information for several frames of a given video.
We empirically find that, despite the simplicity of this approach and the domain gap between image and video data, a zero-shot CLIP significantly outperforms all continual learning methods in the literature on both Kinetics and ActivityNet VCIL setups. Third, we find the core idea of the zero-shot approach (multi-modal contrastive loss) could be used to augment the zero-shot strategy, thus enabling prompting mechanisms, temporal modeling, and replay memories that still rely on a frozen CLIP encoder. The augmented version of our zero-shot baseline sets a new state-of-the-art in every dataset in the vCLIMB benchmark.



% As mentioned before we work over a fully frozen clip encoder. Therefore we use the original clip strategy to generate semantic labels. We classify the video by measuring the distance between the visual and textual embeddings

% Describe how we use it. (We took the Clip textual encoder and fixed it during the whole sequence training. Likewise, . (Nearest Neighbor). We can motivate this in the idea that multi-modal information can help to learn quickly with fewer samples, which is useful when the model learns with limited memory. (Put equations). 

\subsection{PIVOT Model}\label{sec:pivot_model}
% Prompting methods \cite{Wang_2022_CVPR, wang2022dualprompt} have emerged as an alternative to traditional rehearsal methods. While prompting mechanisms have been show effective on drastically reduced memory sizes, they rely on in-distribution pre-training to make suitable prompt selections \cite{Wang_2022_CVPR}. We approach a more general case, where we learn to prompt for video data, while relying exclusively on image domain knowledge-bases.

% We outline a 3 stage process that allows us to effectively train and select prompts for an image encoder on video data. Our prompting strategy allows the image model to be effective in a video task despite having no in-domain pre-training. To the authors best knowledge, this is the first prompting method that can work in the presence of a domain shift. 
Prompting methods \cite{Wang_2022_CVPR, wang2022dualprompt} have emerged as an alternative to traditional rehearsal methods. While prompting mechanisms have been shown effective in drastically reducing memory sizes, they rely on in-distribution pre-training to make suitable prompt selections \cite{Wang_2022_CVPR}. We approach a more general case, where we learn to prompt for video data while relying exclusively on image-language knowledge bases. To this end, we propose PIVOT, a Prompting-based Model for Video Continual Learning. PIVOT leverages CLIP $(f_{sp})$ to encode spatial information and a transformer as temporal encoder $(f_{tp})$ to model the temporal relations essential to understanding actions. Additionally, we define a novel spatial and temporal prompting scheme that captures specific properties of each task to increase the model performance while mitigating the forgetting of previously learned tasks. Figure \ref{fig:model_fig} illustrates the PIVOT pipeline.

% \fch{I think having a figure illustrating this three-step training process would be helpful}
We outline a 3-stage process to effectively train and select prompts for the spatial and temporal dimensions of video data by leveraging extensive image domain pre-training. Despite having no video domain pre-training, our prompting strategy is effective on video classification tasks. To the best of our knowledge, this is the first prompting method that can work in the presence of such a domain shift. 

\paragraph{Out-of-distribution Adaptation.} The first training stage adapts an image pre-trained model to extract video features. Given an input video $\textit{\textbf{v}} \in \mathbb{R}^{T \times H \times W \times C}$, where $T$ is the number of video frames, we utilize CLIP to encode the video frames into meaningful spatial features $ \textit{\textbf{v}}_{sp} = f_{sp}(\textit{\textbf{v}}) \in \mathbb{R}^{T \times D_m}$. 
% Then, we append a $[class]$ token, which aggregates the temporal information of the feature sequence, to the spatial features.
These spatial features are then passed through the temporal encoder where we append a $[class]$ token that aggregates the temporal information of the feature sequence, resulting in the temporal feature of the video $ \textit{\textbf{v}}_{tp} = f_{tp}(\textit{\textbf{v}}_{sp})[class] \in \mathbb{R}^{D_m}$. During this process, the CLIP encoder is completely frozen to avoid any distribution shift. In contrast, the temporal encoder is trained with the current task data $(X_i, Y_i)$. Specifically, we train the temporal encoder following the MCL approach outlined in Section~\ref{sec:mcl}. By using an approach that is informed by the CLIP frozen features, we ensure that the learned features of the temporal model stay consistent with the knowledge of the original image-language model. 
% \JC{The big point here is that using MCL to train the temporal encoder will generate features that are compatible with the language stream of clip, granted these are not clip video features, but are very related to pre-trained clip}

\paragraph{Task-specific Prompt Generation.} After tuning the temporal component of our model, the second training stage aims at learning task-specific prompts. Current prompting methods \cite{Wang_2022_CVPR} would rely on continuously updating a prompt pool along the full task set. Since we can not rely on in-distribution pre-training to update and select prompts, we adopt task-specific prompts that preserve individual task knowledge along the CL process. Essentially, we train a new set of prompts as the data for a new task becomes available, then we append these new prompts into the pre-existent pool. 

%Unlike L2P, we adopt this task-specific prompting scheme to avoid overwriting the previous task knowledge. Even more 

% \JC{We mention MCL like we explained already!}
In addition to maintaining task-specific prompts, we propose to train the prompts and the prompt selector separately. At training time, we optimize the task-specific prompts $P_{n}$ for task $n$ following the MCL approach, while the prompts associated to previous tasks ($P_{n-1} \cup P_{n-2} \cup ... P_{0}$) remain fixed. To address the temporal nature of video data, each task will estimate independent spatial and temporal prompts $P_n = (P_n^{sp}, P_n^{tp})$, where $P_n^{sp} \in \mathbb{R}^{N_p \times L_{sp} \times D_{in}}$ and $P_n^{tp} \in \mathbb{R}^{N_p \times L_{tp} \times D_m}$, $N_p$ is the number of prompts per task,  $L_{sp}$ and $L_{tp}$ are the lengths of spatial and temporal prompts, respectively, and $D_{in}$ is the output dimension of the CLIP input layer $f^e_{sp}$.


%One of the most crucial parts of prompting-based models \cite{Wang_2022_CVPR, wang2022dualprompt} is the prompt selection process. It defines the prompts to use and train. U
\paragraph{Prompt Selection}\label{par:prompts}
Unlike L2P \cite{wang2022dualprompt}, we can not use extensive in-domain knowledge to select the best prompts for each input. To alleviate CLIP's lack of domain comprehension, and thus improve its selection performance, we train the temporal encoder to select the prompts. We first associate each task-specific prompt with the feature set  estimated from the frozen CLIP representations. To this end, we use the feature estimated on the language stream of CLIP, using the labels that belong to each individual task as textual input to the stream, this feature set will define the key $K$ to index a prompt: $\{(K_1, P_1), (K_2, P_2),\dots,(K_n, P_n)\}$, where $K_n \in \mathbb{R}^{M_n \times D_m}$, $M_n$ is the number classes on task $n$, and $D_m$ is the output dimension of CLIP Text encoder. 

We train the temporal encoder to select the corresponding task prompts for each input following a pseudo-classification based on the distance estimated by the MCL. We select the task prompts with the most similar key to the final video representation $\textit{\textbf{v}}_{tp}$. Likewise, once the model selects the prompts, we train the temporal encoder to support them with an MCL. 
% \JC{Cant tell what the final sentence is about}




% \textbf{Task Specific tuning 3}
% we rretrain the teporal layer and use the model wothout promtp, 

% \paragraph{Pseudo Labels for keys}
% \JC{Andres please complete here }

%Explain the enormous challenge of using prompts in the video domain. We do not have extensive in-domain pre-training as in L2P, so we do not have an oracle that can decide with high confidence what prompts the model has been used according to the input. Remember our training stages.


\subsection{PIVOT Forward Pass }\label{sec:classifying_with_pivot}
In Section~\ref{sec:pivot_model}, we outlined the construction and selection of both spatial and temporal prompts. 
Next, we discuss how do we use these prompts during inference.

First, we note that CLIP $f_{sp}$ is based on the ViT architecture, so, it is composed of input layer $f^e_{sp}$ and self-attention layers $f^s_{sp}$. 
Given an input video $v$, we pass it through $f^e_{sp}$, which divides each frame into $L$ patches and encodes them to $\textit{\textbf{v}}_{sp} = f^e_{sp}(\textit{\textbf{v}}) \in \mathbb{R}^{T \times L \times D_{in}}$. We leverage the spatial prompts at this stage, and concatenate $P_n^{sp}$ with $\textit{\textbf{v}}_{sp}$ resulting in $\textit{\textbf{v}}^{e}_{sp}=[P_n^{sp}; \textit{\textbf{v}}_{sp}] \in \mathbb{R}^{T \times (N_pL_{sp}+L) \times D_{in}}$ and pass the extended sequence to the self-attention layers $\textit{\textbf{v}}^{s}_{sp} = f^s_{sp}(\textit{\textbf{v}}^{e}_{sp}) \in \mathbb{R}^{T \times (N_pL_{sp}+L) \times D_{m}}$. Following \cite{Wang_2022_CVPR}, for the final spatial representation we take an average pooling (AvgPool) through the first $N_pL_{sp}$ tokens of $\textit{\textbf{v}}^{s}_{sp}$ resulting in $\textit{\textbf{v}}^{avg}_{sp}\in\mathbb R^{T\times L}$. It is important to note that, we use the same spatial prompt for all frames in a given video.



%Since these encoded features for the $T$ sampled frames from the video represent the visual features of the video,



The previous process results in an embedding vector for each frame that takes into account both the extracted knowledge from CLIP and the learnt spatial prompts.
We then aim at aggregating the information across all frames by leveraging a temporal encoder $f_{tp}$.
Before we do so, we employ the learnt temporal prompts in a similar fashion to the spatial ones.
In particular, we first concatenate $x = [P_n^{tp}; \textit{\textbf{v}}^{avg}_{sp}]$ and then pass it through the temporal encoder followed by an average pooling layer. Formally $\textit{\textbf{v}}_{tp} = AvgPool(f_{tp}(x)[:N_pL_{tp}])  \in \mathbb{R}^{ D_{m}}$.
At last, we use $\textit{\textbf{v}}_{tp}$ as a global feature representation for the input video to classify it with the MCL classifier outlined in Section~\ref{sec:mcl}. 

\subsection{Training PIVOT}\label{sec:training_prompts}
Our training pipeline is divided into three stages for each task in the VCIL setup.
We first train our temporal encoder to correctly classify input data within the current task.
Then, we leverage the knowledge of both CLIP and the trained temporal encoder to learn per task learnable tokens, \ie prompts.
At last, We fine tune the temporal encoder to select and leverage the learnt prompts to enhance the performance and reduce forgetting.
It is worth mentioning that we freeze CLIP throughout the entire training process. 
% \fch{align the names of the paragraphs below with those defined earlier i.e. out-of-distribution training, task-specific prompt gen, ...}

\paragraph{First Stage: Out-of-distribution Adaptation.} 
In this stage, we want to align the temporal encoder with the extracted representation of a given video from CLIP.
To do so, we train our temporal encoder to correctly classify a given video based on the extracted features from CLIP with an MCL loss.
Let $\theta_{tp}$ be the learnable parameters for $f_{tp}$, we seek to minimize the loss for the $n^{th}$ task:
% It is training using only the current task data. In this step, we train the temporal layer for the current task.
% Overall, we seek to minimize the loss:  
\begin{equation}\label{eq:first_stage_training}
\min_{\theta_{tp}} \mathbb E_{(v, y)\sim (X_n, Y_n)}\left[ \mathcal{L}\left(f_{tp}(f_{sp}(\textit{\textbf{v}})), \textit{\textbf{y}}\right)\right],
\end{equation}
where \textit{\textbf{y}} is the representation of the class label of \textit{\textbf{v}} obtained with the CLIP text encoder, $\mathcal L$ is the MCL loss, and $(X_n, Y_n)$ is the data distribution for the $n^{th}$ task.
We note here that relying solely on Eq.~\eqref{eq:first_stage_training} for training might result in forgetting previously learnt tasks.


\paragraph{Second Stage: Task-specific Prompt Generation.} 
In this stage, we leverage the learnt knowledge of the temporal encoder to learn meaningful prompts that are specific for task $n$.
To that end, we freeze the temporal encoder during this stage.
We randomly initialize a set of prompts for task $n$ denoted as $P_n = (P_n^{sp}, P_n^{tp})$.
We include $P_n$ in the forward propagation of our pipeline as discussed in Section~\ref{sec:classifying_with_pivot}.
We then learn the prompts $P_n$ by minimizing the following loss:
% In this step, the specific task prompts, both spatial and temporal task prompts are trained using the current task data. 
\begin{equation}\label{eq:learning_prompts}
\min_{P_{sp}, P_{tp}}  \mathbb E_{(v, y)\sim (X_n, Y_n)}\left[\mathcal{L}\left(f_{tp}(f_{sp}(\textit{\textbf{v}}, P^{sp}_n),P^{tp}_n), \textit{\textbf{y}}\right)\right].
\end{equation}
Note that Equation~\ref{eq:learning_prompts} aims at aligning the learnable prompts with the knowledge of both CLIP and the learnt temporal encoder for the same task.
This is accomplished through solely relying on $P_n$ to correctly classify a given video.
We note here that we freeze the prompts for a given task while learning prompts for other tasks.

\paragraph{Third Stage: Prompt Selection.}
In the last training stage, we fine tune the temporal encoder to better leverage the learnt prompts.
This is accomplished through minimizing the combined MCL loss from Equations~\ref{eq:first_stage_training} and \ref{eq:learning_prompts} through the following:

\begin{equation}
\begin{split}
\min_{\theta_{tp}} \mathbb E_{(v, y)\sim (X_n, Y_n)}\big[ \mathcal{L}(f_{tp}(f_{sp}(\textit{\textbf{v}}, P_{sp}),P_{tp}), \textit{\textbf{y}}) \\ +  \mathcal{L}(f_{tp}(f_{sp}(\textit{\textbf{v}})), \textit{\textbf{y}}) \big].
\end{split}
\label{eq:last_step}
\end{equation}

It is worth mentioning that the last training step in Eq.~\eqref{eq:last_step} aligns the parameters of the temporal encoder to solidify the knowledge of a given task by correctly classifying the input based on the selected prompts in addition to the input. 
This will reduce forgetting previously learnt tasks as their corresponding prompts are frozen.

Next, we analyze the effectiveness of our approach empirically in the vCLIMB benchmark.

% The last training step aims to train the temporal layer to select the corresponding set of prompts for each specific input. Moreover, it is trained to use those prompts to get a better performance in all tasks. In this step, we seek to minimize the Eq~\ref{eq:last_step}, using the current task data and the memory data. 



% Overall, we seek to minimize the loss:  

% \begin{equation}
% \begin{split}
% \min_{P_{sp}, P_{tp}, f_{tp}} L_{MCL}(f_{tp}(f_{sp}(\textit{\textbf{v}}, P_{sp}),P_{tp}), \textit{\textbf{y}}) \\ +  L_{MCL}(f_{tp}(f_{sp}(\textit{\textbf{v}})), \textit{\textbf{y}})
% \end{split}
% \end{equation}
% where \textit{\textbf{y}} is the representation of the class label of \textit{\textbf{v}} obtained with the CLIP text encoder.

%Describe how we leverage the clip knowledge and extend it to video using a transformer encoder to encode video targets. 


% \subsection{Temporal Modeling}
% \JC{This section will be deleted}

% We further propose aggregating the temporal information via training continually a temporal transformer showing consistent improvement over the zero-shot approach of deploying CLIP.
% We equip our approach with a learnable prompts module for both the spatial and temporal modulations.
% The module incrementally learns a meaningful space for the prompts, and using it further boosts the performance by 9\%

% \begin{enumerate}
%     \item Until now, our best model is the CLIP + Temp + MCL. This method leverages extensive knowledge of the clip's textual encoder to train our method. It is always used fixed to avoid forgetting.
%     \item For the Temp aggregation method, we use a transformer encoder and consider a sequence of 8 frames per video. 
%     \item The big challenge of using prompts is the selection process because we do not have extensive in-domain pre-training as in L2P. Likewise, it is tough to think in temporal prompts because we do not have general temporal knowledge to modulate.
% \end{enumerate}

% Describe our CL setup and the scenarios we used (vCLIMB datasets and tasks). Metrics, etc.










% Given an input video $\textit{\textbf{v}}$, we pass it through $f^e_{sp}$, which divides each frames in $L$ patches (including the $[class]$ token) and encode them, $\textit{\textbf{v}}^e_{sp} = f^e_{sp}(\textit{\textbf{v}}) \in \mathbb{R}^{T \times L \times D_{in}}$. Then, we concatenate the $P_n^{sp}$ with the $\textit{\textbf{v}}^{e}_{sp} =[P_n^{sp}; \textit{\textbf{v}}^e_{sp}] \in \mathbb{R}^{T \times (N_pL_{sp}+L) \times D_{in}}$ and pass the extended sequence to the self-attention layers $\textit{\textbf{v}}^{e}_{sp} = f^s_{sp}(\textit{\textbf{v}}^{e}_{sp}) \in \mathbb{R}^{T \times (N_pL_{sp}+L) \times D_{m}}$. Following \cite{Wang_2022_CVPR}, for the final spatial representation $\textit{\textbf{v}}_{sp}$ we take an average pooling (AvgPool) through the first $N_pL_{sp}$ tokens of $v^{e}_{sp}$. It is important to note that we consider the same spatial prompt for all frames in a video. Likewise, we add the corresponding temporal prompt to the spatial video representation $\textit{\textbf{v}}_{sp} =[P_n^{tp}; \textit{\textbf{v}}_{sp}] \in \mathbb{R}^{(N_pL_{tp}+T) \times D_{m}}$. Then, we feed the extended temporal sequences to the temporal encoder and consider the $N_pL_{tp}$ temporal prompt tokens to compute the final video representation $\textit{\textbf{v}}_{tp} = AvgPool(f_{tp}(\textit{\textbf{v}}_{sp})[:N_pL_{tp}])  \in \mathbb{R}^{ D_{m}}$. 


% \subsection{Learning Video CIL representations with PIVOT}
